Search for Higgs boson pair production in the $WW^{(*)}WW^{(*)}$ decay channel using ATLAS data recorded at $\sqrt{s}=13$ TeV

A search for a pair of neutral, scalar bosons with each decaying into two $W$ bosons is presented using 36.1 fb$^{-1}$ of proton-proton collision data at a centre-of-mass energy of 13 TeV recorded with the ATLAS detector at the Large Hadron Collider. This search uses three production models: non-resonant and resonant Higgs boson pair production and resonant production of a pair of heavy scalar particles. Three final states, classified by the number of leptons, are analysed: two same-sign leptons, three leptons, and four leptons. No significant excess over the expected Standard Model backgrounds is observed. An observed (expected) 95% confidence-level upper limit of 160 (120) times the Standard Model prediction of non-resonant Higgs pair production cross-section is set from a combined analysis of the three final states. Upper limits are set on the production cross-section times branching ratio of a heavy scalar $X$ decaying into a Higgs boson pair in the mass range of 260 GeV $\le m_X \le$ 500 GeV and the observed (expected) limits range from 9.3 (10) pb to 2.8 (2.6) pb. Upper limits are set on the production cross-section times branching ratio of a heavy scalar $X$ decaying into a pair of heavy scalars $S$ for mass ranges of 280 GeV $\le m_X \le$ 340 GeV and 135 GeV $\le m_S \le$ 165 GeV and the observed (expected) limits range from 2.5 (2.5) pb to 0.16 (0.17) pb.

==> HIGG-2016-24-PAPER-auxmat.tex <==

\part*{Auxiliary material}
\addcontentsline{toc}{part}{Auxiliary material}
\label{sec:Auxiliary}

\input{aux/vars_preselection_2l}

\clearpage

\input{aux/vars_preselection_3l}

\input{aux/vars_WZCR_3l}

\clearpage

\input{aux/vars_preselection_4l}

\input{aux/vars_ZZCR_4l}

\input{aux/vars_final_4l}

\clearpage

\input{tables/yields_2l}

\clearpage

\input{tables/yields_3l}

\clearpage

\input{tables/yields_4l}

\clearpage

\input{aux/yields}

\clearpage

\input{tables/systematics}

\clearpage

\input{tables/limits_resonant}


==> tables/limits_resonant.tex <==


\begin{table}[!ht]
  \centering
  \begin{tabular}{c S[table-format=3.0] S[table-format=2.2] S[table-format=2.2] S[table-format=2.2] S[table-format=2.2]}
    \toprule
    & \multicolumn{1}{c}{\multirow{2}{*}{Non-res./SM}} & \multicolumn{1}{c}{$m_X = 260$~GeV} & \multicolumn{1}{c}{$m_X = 300$~GeV} & \multicolumn{1}{c}{$m_X = 400$~GeV} & \multicolumn{1}{c}{$m_X = 500$~GeV} \\
    & & [pb] &  [pb] &  [pb] &  [pb]  \\
    \midrule
    \midrule
    Expected: 2 leptons &140 & 37 & 30 & 12 & 3.4 \\
    \midrule
    Expected: 3 leptons & 270 & 23 & 24 & 11 & 7.5 \\
    \midrule
    Expected: 4 leptons & 400 & 13 & 13 & 13 & 10 \\
    \midrule
    \midrule
    Expected & 120 & 9.9 & 10 & 6.7 & 2.6 \\
    \midrule
    +2$\sigma$ & 230 & 21 & 21 & 14 & 5.8 \\
    \midrule
    +1$\sigma$ & 170 & 15 & 15 & 9.7 & 3.9 \\
    \midrule
    -1$\sigma$ & 83 & 7.1 & 7.2 & 4.9 & 1.9 \\
    \midrule
    -2$\sigma$ & 62 & 5.3 & 5.4 & 3.6 & 1.4 \\
    \midrule
    \midrule
    Observed & 160 & 9.3 & 8.5 & 5.3 & 2.8 \\
    \bottomrule
  \end{tabular}
  \caption{Summary of the 95\% CL upper limits on cross-section of SM non-resonant $HH$ production and on 
                cross-section times branching ratio of resonant $HH$ production.  Expected limits are shown for each 
                channel as well as the combination of the channels. The $\pm1\sigma$ and $\pm1\sigma$ boundaries 
                of the expected limits are also shown for the combination of channels.  The limits for non-resonant 
                production are given in terms of the ratio to the SM prediction.  The limits for resonant production are 
                given in units of pb.}
  \label{tab:limit-comb}
\end{table}

\begin{table}[!ht]
  \centering
  \begin{tabular}{ccccc}
    \toprule
    & $m_X = 280$~GeV & $m_X = 300$~GeV & $m_X = 320$~GeV & $m_X = 340$~GeV \\
         & [pb] &  [pb] &  [pb] &  [pb]  \\
    \midrule
    \midrule
    Expected: 2 leptons & 6.1 & 5.7 & 5.9 & 4.9 \\
    \midrule
    Expected: 3 leptons & 4.1 & 4.7 & 5.2 & 3.9 \\
    \midrule
    Expected: 4 leptons & 3.2 & 3.2 & 3.6 & 3.6 \\
    \midrule
    \midrule
    Expected & 2.1 & 2.3 & 2.5 & 2.2 \\
    \midrule
    +2$\sigma$ & 4.6 & 4.9 & 5.1 & 4.5 \\
    \midrule
    +1$\sigma$ & 3.1 & 3.4 & 3.6 & 3.2 \\
    \midrule
    -1$\sigma$ & 1.5 & 1.7 & 1.8 & 1.6 \\
    \midrule
    -2$\sigma$ & 1.1 & 1.3 & 1.3 & 1.2 \\
    \midrule
    \midrule
    Observed & 1.8 & 2.2 & 2.4 & 2.5 \\
    \bottomrule
  \end{tabular}
  \caption{Summary of the 95\% CL upper limits on cross-section times branching ratio of $X\rightarrow SS$ production with $m_S=135$~GeV.  Expected limits are shown for each channel as well as the combination of the channels.  The $\pm1\sigma$ and $\pm1\sigma$ boundaries of the expected limits are also shown for the combination of channels.  The limits are given in units of pb.}
  \label{tab:limit-comb-SS-mX}
\end{table}

\begin{table}[!ht]
  \centering
  \begin{tabular}{c S[table-format=1.2] S[table-format=1.2] S[table-format=1.3]}
    \toprule
    & \multicolumn{1}{c}{$m_{S} = 145$~GeV} & \multicolumn{1}{c}{$m_{S} = 155$~GeV} & \multicolumn{1}{c}{$m_{S} = 165$~GeV} \\
        &  [pb] &  [pb] &  [pb]  \\
    \midrule
    \midrule
    Expected: 2 leptons & 1.5 & 0.69 & 0.37 \\
    \midrule
    Expected: 3 leptons & 1.6 & 0.65 & 0.25 \\
    \midrule
    Expected: 4 leptons & 1.4 & 0.66 & 0.37 \\
    \midrule
    \midrule
    Expected & 0.82 & 0.38 & 0.17 \\
    \midrule
    +2$\sigma$ & 1.7 & 0.75 & 0.35 \\
    \midrule
    +1$\sigma$ & 1.2 & 0.53 & 0.25 \\
    \midrule
    -1$\sigma$ & 0.59 & 0.27 & 0.13 \\
    \midrule
    -2$\sigma$ & 0.44 & 0.20 & 0.094 \\
    \midrule
    \midrule
    Observed & 0.66 & 0.35 & 0.16 \\
    \bottomrule
  \end{tabular}
  \caption{Summary of the 95\% CL upper limits on cross-section times branching ratio of $X\rightarrow SS$ production with $m_X=340$~GeV.  Expected limits are shown for each channel as well as the combination of the channels.  The $\pm1\sigma$ and $\pm1\sigma$ boundaries of the expected limits are also shown for the combination of channels.  The limits are given in units of pb.}
  \label{tab:limit-comb-SS-mS}
\end{table}


==> tables/systematics.tex <==

\begin{table}[!ht]
  \centering
  \begin{tabular}{l S[table-format=1.3] S[table-format=1.3] S[table-format=1.3] S[table-format=1.3] S[table-format=1.3]}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Source}} & \multicolumn{1}{c}{Non-res.} & \multicolumn{1}{c}{$m_{X}=260$~GeV} & \multicolumn{1}{c}{$m_{X}=300$~GeV} & \multicolumn{1}{c}{$m_{X}=400$~GeV} & \multicolumn{1}{c}{$m_{X}=500$~GeV} \\
    & [\%] & [\%]& [\%]& [\%]& [\%] \\
    \midrule
Electron calib.	&2.6	&0.7	&0.4	&0.6	&3.0\\
\midrule
Electron eff.	&2.9	&3.1	&2.8	&2.2	&2.2\\
\midrule

Fake estimate	& 41.9	&38.0	&30.7	& 53.5	& 40.0\\
\midrule

Theory	&23.3	&35.6	&27.9	&25.9	&24.1\\

\midrule
Jet calib.	&44.9	&30.3	&54.8	&44.3	&28.7\\
\midrule

 Luminosity	&6.2	&7.0	&9.5	&6.0	&5.0\\
\midrule
\met	&3.1	&3.1	&4.2	&1.3	&1.2\\
\midrule

Muon eff. &5.5	&2.1	&2.9	&2.0	& 2.1\\
\midrule
Pileup&4.9	&2.6	&3.3	&7.3	& 1.2\\
\midrule
Flavour tagging	&7.7	&2.8	&6.4	&6.4	&6.7\\
\midrule
MC statistics&21.1	&15.8	&17.7&16.8&21.0\\
\midrule
All syst.&70.5	&63.4	&72.3&77.1&59.6\\
\midrule
Stat. only& 70.9	&77.0	&68.7&63.6&80.3\\
    \bottomrule
  \end{tabular}
  \caption{The impact of systematic uncertainties on the combined cross-section limit for SM non-resonant $HH$ production 
                and on the combined cross-section times branching ratio limits for resonant $HH$ production. All values are 
                expressed as percentage.  The impact of each systematic is defined as 
                $\sqrt{\mu_{\text{syst}+\text{stat}}^2-\mu_\text{stat}^2}/\mu_{\text{allsyst}+\text{stat}}$ where $\mu_\text{stat}$ 
                is the expected limit considering only statistical uncertainties, $\mu_{\text{syst}+\text{stat}}$ is the expected 
                limit considering statistical uncertainties and a single systematic uncertainty, and $\mu_{\text{allsyst}+\text{stat}}$ 
                is the expected limit considering statistical and all systematic uncertainties.  The impact of the statistical uncertainty 
                is defined as $\mu_\text{stat}/\mu_{\text{allsyst}+\text{stat}}$.}
  \label{table:sys1}
\end{table}


\begin{table}[!ht]
  \centering
  \begin{tabular}{l S[table-format=1.4,table-comparator = true] S[table-format=1.4,table-comparator = true] S[table-format=1.4,table-comparator = true] S[table-format=1.4,table-comparator = true]}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Source}} & \multicolumn{1}{c}{$m_{X}=280$~GeV} & \multicolumn{1}{c}{$m_{X}=300$~GeV} & \multicolumn{1}{c}{$m_{X}=320$~GeV} & \multicolumn{1}{c}{$m_{X}=340$~GeV} \\
& [\%]& [\%]& [\%]& [\%] \\
    \midrule
 Electron calib.	&4.3	&0.8	&0.0	&3.4\\
\midrule
Electron eff.	&2.6	&3.1	&3.4	&3.0\\
\midrule

Fake estimate	& 37.4	&46.1	&47.6	& 42.5\\
\midrule

Theory	&30.3	&31.0	&30.2	&32.1\\

\midrule
Jet calib.	&38.3	&43.9	&48.5	&50.8\\
\midrule

 Luminosity	&7.4	&7.2	&7.3	&8.0\\
\midrule
\met	&2.5	&3.2	&3.8	&3.6\\
\midrule

Muon eff.&1.9	&1.9	&1.1	&1.9\\
\midrule
Pileup &2.3	&5.2	&7.2	&4.4\\
\midrule
Flavour tagging	&4.5	&4.7	&5.1	&7.1	\\
\midrule
MC statistics&16.5	&17.0	&17.6&17.3\\
\midrule
All syst.&65.1	&74.0	&77.8&76.9\\
\midrule
Stat. only& 76.0	&67.2	&62.8&64.0\\
    \bottomrule
  \end{tabular}
  \caption{The impact of systematic uncertainties on the combined cross-section times branching ratio limits for 
                $X\rightarrow SS$ production with $m_S = 135$~GeV. All values are expressed as percentage.  The 
                impact of each systematic is defined as 
                $\sqrt{\mu_{\text{syst}+\text{stat}}^2-\mu_\text{stat}^2}/\mu_{\text{allsyst}+\text{stat}}$ where $\mu_\text{stat}$ 
                is the expected limit considering only statistical uncertainties, $\mu_{\text{syst}+\text{stat}}$ is the expected 
                limit considering statistical uncertainties and a single systematic uncertainty, and $\mu_{\text{allsyst}+\text{stat}}$ 
                is the expected limit considering statistical and all systematic uncertainties.  The impact of the statistical 
                uncertainty is defined as $\mu_\text{stat}/\mu_{\text{allsyst}+\text{stat}}$.}
  \label{table:sys2}
\end{table}

\begin{table}[!ht]
  \centering
  \begin{tabular}{l S[table-format=1.4,table-comparator = true] S[table-format=1.4,table-comparator = true] S[table-format=1.4,table-comparator = true]}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Source}} & \multicolumn{1}{c}{$m_{S}=145$~GeV} & \multicolumn{1}{c}{$m_{S}=155$~GeV} & \multicolumn{1}{c}{$m_{S}=165$~GeV} \\
& [\%]& [\%]& [\%] \\
    \midrule
 Electron calib.	&5.1	&5.0	&3.5	\\
\midrule
Electron eff.	&2.2	&2.4	&2.8\\
\midrule

Fake estimate	& 48.6	&51.4	&52.1\\
\midrule

Theory	&28.5	&27.6	&24.6\\

\midrule
Jet calib.	&47.1	&48.9	&48.9\\
\midrule

 Luminosity	&7.6	&7.6	&7.3	\\
\midrule
\met	&1.9	&2.3	&2.1\\
\midrule

Muon eff.&1.6	&1.5	&1.2\\
\midrule
Pileup &1.7	&2.5	&4.2\\
\midrule
Flavour tagging	&7.1	&7.0	&6.7	\\
\midrule
MC statistics&16.4	&17.4	&17.9\\
\midrule
All syst.&76.3	&79.1	&78.6\\
\midrule
Stat. only& 64.7	&61.2	&61.8\\  
    \midrule
  \end{tabular}
  \caption{The impact of systematic uncertainties on the combined cross-section times branching ratio limits for 
                $X\rightarrow SS$ production with $m_X = 340$~GeV. All values are expressed as percentage.  The 
                impact of each systematic is defined as 
                $\sqrt{\mu_{\text{syst}+\text{stat}}^2-\mu_\text{stat}^2}/\mu_{\text{allsyst}+\text{stat}}$ where $\mu_\text{stat}$ 
                is the expected limit considering only statistical uncertainties, $\mu_{\text{syst}+\text{stat}}$ is the expected 
                limit considering statistical uncertainties and a single systematic uncertainty, and $\mu_{\text{allsyst}+\text{stat}}$ 
                is the expected limit considering statistical and all systematic uncertainties.  The impact of the statistical 
                uncertainty is defined as $\mu_\text{stat}/\mu_{\text{allsyst}+\text{stat}}$.}
  \label{table:sys3}
\end{table}


==> tables/yields_2l.tex <==

\begin{table}[!ht]
  \centering
  \begin{tabular}{cc S[table-format=3.2]@{$\pm$}S[table-format=3.2] S[table-format=1.4]@{$\pm$}S[table-format=2.3] S[table-format=1.0]}
    \toprule
    $m_X$ & Category & \multicolumn{2}{c}{Background} & \multicolumn{2}{c}{Expected Signal} & \multicolumn{1}{c}{Observed} \\
    \midrule
    \midrule
    \multirow{3}{*}[-6pt]{Non-res.}
    & $ee$ & 29 & 10 & 0.028 & 0.004 & 35 \\
    \cmidrule{2-7}
    & $\mu\mu$ &8.1 & 2.5 & 0.034 & 0.004 & 4 \\
    \cmidrule{2-7}
    & $e\mu$ & 11.1 & 2.2 & 0.049 & 0.005 & 18 \\
    \midrule
    \midrule
    \multirow{3}{*}[-6pt]{260~GeV}
    & $ee$ & 48 & 14 & 0.44 & 0.14 & 62 \\
    \cmidrule{2-7}
    & $\mu\mu$ & 24 & 9 & 0.54 & 0.24 & 17 \\
    \cmidrule{2-7}
    & $e\mu$ & 71 & 14 & 0.99 & 0.23 & 70 \\
    \midrule
    \midrule
    \multirow{3}{*}[-6pt]{300~GeV}
    & $ee$ &67 & 19 & 0.61 & 0.20 & 89  \\
    \cmidrule{2-7}
    & $\mu\mu$ & 125 & 44 & 1.5 & 0.5 & 74  \\
    \cmidrule{2-7}
    & $e\mu$ & 132 & 23 & 2.0 & 0.4 & 144  \\
    \midrule
    \midrule
    \multirow{3}{*}[-6pt]{400~GeV}
    & $ee$ & 35 & 11 & 0.81 & 0.23 & 46  \\
    \cmidrule{2-7}
    & $\mu\mu$ & 28 & 8 & 1.3 & 0.3 & 19  \\
    \cmidrule{2-7}
    & $e\mu$ &45 & 8 & 2.2 & 0.8 & 57  \\
    \midrule
    \midrule
    \multirow{3}{*}[-6pt]{500~GeV}
    & $ee$ & 9.3 & 3.0 & 0.85 & 0.09 &14 \\
    \cmidrule{2-7}
    & $\mu\mu$ & 8.0 & 2.5 & 1.4 & 0.3 & 4 \\
    \cmidrule{2-7}
    & $e\mu$ & 9.0 & 1.7 & 1.9 & 0.3 & 10 \\
    \bottomrule
  \end{tabular}
  \caption{Expected and observed yields after all selection criteria for the non-resonant $HH$ and resonant 
                $X\rightarrow HH$ searches in the two lepton channel.  The non-resonant signal is assumed to 
                have a cross-section of 33.4~fb and the resonant signals are assumed to have a cross-section of 
                1~pb.  The $HH\rightarrow4W\rightarrow\ell^\pm\ell^\pm$+jets branching ratio is assumed to be 
                $4.4\times10^{-3}$.  Systematic uncertainties in the signal and background yields are shown.}
  \label{tab:yields-2l-hh}
\end{table}

\begin{table}[!ht]
  \centering
\begin{tabular}{l S[table-format=1.2]@{$\pm$}S[table-format=2.1] 
                          S[table-format=1.2]@{$\pm$}S[table-format=2.1] 
                          S[table-format=1.2]@{$\pm$}S[table-format=2.1] 
                          S[table-format=1.2]@{$\pm$}S[table-format=2.1] 
                          S[table-format=2.2]@{$\pm$}S[table-format=2.1] 
                          S[table-format=2.1]@{$\pm$}S[table-format=2.0] 
                          S[table-format=2.1]@{$\pm$}S[table-format=2.0]}
\toprule
$m_X$ & \multicolumn{2}{c}{280 GeV} & \multicolumn{2}{c}{300 GeV} & \multicolumn{2}{c}{320 GeV} & \multicolumn{2}{c}{340 GeV} & \multicolumn{2}{c}{340 GeV} & \multicolumn{2}{c}{340 GeV} & \multicolumn{2}{c}{340 GeV} \\
$m_S$ & \multicolumn{2}{c}{135 GeV} & \multicolumn{2}{c}{135 GeV} & \multicolumn{2}{c}{135 GeV} & \multicolumn{2}{c}{135 GeV} & \multicolumn{2}{c}{145 GeV} & \multicolumn{2}{c}{155 GeV} & \multicolumn{2}{c}{165 GeV} \\
\midrule
\midrule
& \multicolumn{12}{c}{Expected Signal} \\
\midrule
    $ee$&1.9 & 0.3&2.1 & 0.4 & 2.0 & 0.3&2.2 & 0.4& 7.2 & 1.2 & 14 & 2 &26 & 4\\
$\mu\mu$&4.4 & 0.7& 4.3 & 0.6& 4.0 & 0.7&4.3 & 0.6& 15 & 2 & 32 & 4&57 & 8\\
  $e\mu$&5.2 & 0.9 & 5.5 & 0.7& 5.4 & 0.7& 5.6 & 0.7& 17 & 2 & 36 & 5&70 & 10\\
\midrule
\midrule
& \multicolumn{12}{c}{Background} \\
&\multicolumn{6}{c}{$m_X < 340$~GeV selection}&\multicolumn{8}{c}{$m_X = 340$~GeV selection} \\
\midrule
$ee$&\multicolumn{6}{c}{38 $\pm$ 11}&\multicolumn{8}{c}{44 $\pm$ 15} \\
$\mu\mu$&\multicolumn{6}{c}{66 $\pm$ 25}&\multicolumn{8}{c}{62 $\pm$ 21} \\
$e\mu$&\multicolumn{6}{c}{70 $\pm$ 13}&\multicolumn{8}{c}{53 $\pm$ 10} \\
\midrule
\midrule
& \multicolumn{12}{c}{Observed} \\
&\multicolumn{6}{c}{$m_X < 340$~GeV selection}&\multicolumn{8}{c}{$m_X = 340$~GeV selection} \\
\midrule
$ee$&\multicolumn{6}{c}{50}&\multicolumn{8}{c}{51} \\
$\mu\mu$&\multicolumn{6}{c}{46}&\multicolumn{8}{c}{38} \\
$e\mu$&\multicolumn{6}{c}{62}&\multicolumn{8}{c}{64} \\
\bottomrule
\end{tabular}
\caption{Expected and observed yields after all selection criteria for the $X\rightarrow SS$ searches 
              in the two lepton channel. The signals are assumed to have a cross-section of 
              1~pb. The $SS\rightarrow4W\rightarrow\ell^\pm\ell^\pm$+jets branching ratio depends on 
              $m_S$ and ranges from $1.5\times10^{-2}$ to $8.8\times10^{-2}$.  Systematic uncertainties 
              in the signal and background yields are shown.  A single set of selection criteria is applied to 
              all signal samples with $m_X < 340$~GeV and another set of selection criteria is applied to 
              all signal samples with $m_X = 340$~GeV.}
  \label{tab:yields-2l-HSS}
\end{table}


==> tables/yields_3l.tex <==


\begin{table}[!ht]
  \centering
  \begin{tabular}{cl S[table-format=1.3]@{$\pm$}S[table-format=2.2] S[table-format=1.4]@{$\pm$}S[table-format=2.3] S[table-format=1.0]}
    \toprule
    $m_X$ & \multicolumn{1}{c}{Category} & \multicolumn{2}{c}{Background} & \multicolumn{2}{c}{Expected Signal} & \multicolumn{1}{c}{Observed} \\
    \midrule
    \midrule
    \multirow{2}{*}[-2pt]{Non-res.}
    & $N_\text{SFOS} = 0$ & 1.00 & 0.69 & 0.011 & 0.005 & 3 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 4.3 & 3.8 & 0.033 & 0.010 & 8 \\
    \midrule
    \midrule
    \multirow{2}{*}[-2pt]{260~GeV}
    & $N_\text{SFOS} = 0$ & 0.70 & 0.52 & 0.082 & 0.046 & 0 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 5.7 & 2.2 & 0.252 & 0.043 & 8 \\
    \midrule
    \midrule
    \multirow{2}{*}[-2pt]{300~GeV}
    & $N_\text{SFOS} = 0$ & 0.63 & 0.12 & 0.084 & 0.010 & 0 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 5.87 & 0.93 & 0.233 & 0.018 & 7 \\
    \midrule
    \midrule
    \multirow{2}{*}[-2pt]{400~GeV}
    & $N_\text{SFOS} = 0$ & 2.2 & 1.1 & 0.26 & 0.11 & 1 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 9.5 & 4.5 & 0.69 & 0.26 & 7 \\
    \midrule
    \midrule
    \multirow{2}{*}[-2pt]{500~GeV}
    & $N_\text{SFOS} = 0$ & 0.23 & 0.13 & 0.36 & 0.22 & 2 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 3.4 & 1.6 & 0.88 & 0.51 & 1 \\
    \bottomrule
  \end{tabular}
  \caption{Expected and observed yields after all selection criteria for the non-resonant $HH$ and resonant 
                $X\rightarrow HH$ searches in the three lepton channel.  The non-resonant signal is assumed to 
                have a cross-section of 33.4~fb and the resonant signals are assumed to have a cross-section of 
                1~pb.  The $HH\rightarrow4W\rightarrow3\ell$+jets branching ratio is assumed to be $4.2\times10^{-3}$. 
                Systematic uncertainties in the signal and background yields are shown.}
  \label{tab:yields-3l-hh}
\end{table}

\begin{table}[!ht]
  \centering
  \begin{tabular}{cl S[table-format=1.3]@{$\pm$}S[table-format=2.2] S[table-format=2.3]@{$\pm$}S[table-format=2.3] S[table-format=1.0]}
    \toprule
    $m_X$/$m_S$ & \multicolumn{1}{c}{Category} & \multicolumn{2}{c}{Background} & \multicolumn{2}{c}{Expected Signal} & \multicolumn{1}{c}{Observed} \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{280~GeV  \\ 135~GeV}}
    & $N_\text{SFOS} = 0$ & 0.41 & 0.31 & 0.41 & 0.16 & 0 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 6.7 & 2.2 & 1.37 & 0.31 & 7 \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{300~GeV \\ 135~GeV}}
    & $N_\text{SFOS} = 0$ & 2.0 & 1.1 & 0.66 & 0.20 & 1 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 12.7 & 5.2 & 1.88 & 0.38 & 17 \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{320~GeV \\ 135~GeV}}
    & $N_\text{SFOS} = 0$ & 2.2 & 1.2 & 0.64 & 0.21 & 1 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 8.6 & 3.7 & 1.52 & 0.52 & 15 \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{340~GeV \\ 135~GeV}}
    & $N_\text{SFOS} = 0$ & 1.15 & 0.64 & 0.71 & 0.25 & 1 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 5.5 & 3.6 & 1.29 & 0.26 & 9 \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{340~GeV \\ 145~GeV}}
    & $N_\text{SFOS} = 0$ & 2.3 & 1.4 & 2.16 & 0.65 & 0 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 10.7 & 4.1 & 4.26 & 0.94 & 13 \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{340~GeV \\ 155~GeV}}
    & $N_\text{SFOS} = 0$ & 2.5 & 1.4 & 4.8 & 1.2 & 1 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 10.4 & 3.8 & 11.5 & 1.9 & 13 \\
    \midrule
    \midrule
    \multirow{2}{*}[-3pt]{\shortstack{340~GeV \\ 165~GeV}}
    & $N_\text{SFOS} = 0$ & 2.5 & 1.4 & 13.9 & 2.6 & 1 \\
    \cmidrule{2-7}
    & $N_\text{SFOS} = \text{1,2}$ & 14.7 & 5.9 & 33.4 & 4.8 & 19 \\
    \bottomrule
  \end{tabular}
  \caption{Expected and observed yields after all selection criteria for the $X\rightarrow SS$ searches in the three 
                lepton channel. The signals are assumed to have a cross-section of 1~pb.  The $SS\rightarrow4W\rightarrow3\ell$+jets 
                branching ratio depends on $m_S$ and ranges from $1.5\times10^{-2}$ to $8.5\times10^{-2}$.  Systematic 
                uncertainties in the signal and background yields are shown.}
  \label{tab:yields-3l-HSS}
\end{table}



==> tables/yields_4l.tex <==

\begin{table}[!ht]
  \centering
  \begin{tabular}{r@{ = }l c c c c}
    \toprule
    \multicolumn{2}{c}{\multirow{2}{*}[-2pt]{Sample}}
    & \multicolumn{2}{c}{$N_\text{SFOS} = \text{0,1}$} & \multicolumn{2}{c}{$N_\text{SFOS} = 2$} \\
    \cmidrule{3-6}
    \multicolumn{2}{c}{} & $m_{4\ell}<180$~GeV & $m_{4\ell}>180$~GeV & $m_{4\ell}<180$~GeV & $m_{4\ell}>180$~GeV \\
    
    \midrule
    \midrule
    
    \multicolumn{2}{c}{Non-res.} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.0053 & 0.0010
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.0100 & 0.0017
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.0018 & 0.0005
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.0046 & 0.0009
    \end{tabular} \\
    
    \midrule
    
    $m_X$ & 260~GeV &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      4.47 & 0.63
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.0011 & 0.0012
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      2.00 & 0.31
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.00 & 0.00
    \end{tabular} \\
    
    \midrule
    
    $m_X$ & 300~GeV &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      4.48 & 0.65
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.66 & 0.14
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      1.58 & 0.25
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.214 & 0.048
    \end{tabular} \\
    
    \midrule
    
    $m_X$ & 400~GeV &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      2.62 & 0.38
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      3.57 & 0.51
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.85 & 0.14
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      1.45 & 0.23
    \end{tabular} \\
    
    \midrule
    
    $m_X$ & 500~GeV &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      1.10 & 0.18
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      4.49 & 0.63
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      0.392 & 0.078
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      1.86 & 0.29
    \end{tabular} \\
    
    \midrule
    
    $m_X$ & 280~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.48 & 0.68
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.022 & 0.011
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.79 & 0.31
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.0031 & 0.0034
      \end{tabular}
    } \\
    
    $m_S$ & 135~GeV \\
    
    \midrule
    
    $m_X$ & 300~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.52 & 0.68
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.286 & 0.072
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.73 & 0.30
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.105 & 0.032
      \end{tabular}
    } \\
    $m_S$ & 135~GeV \\
    
    \midrule
    
    $m_X$ & 320~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.44 & 0.69
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.75 & 0.15
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.69 & 0.30
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.289 & 0.071
      \end{tabular}
    } \\
    $m_S$ & 135~GeV \\
    
    \midrule
    
    $m_X$ & 340~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.17 & 0.65
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.68 & 0.31
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.50 & 0.27
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.52 & 0.11
      \end{tabular}
    } \\
    $m_S$ & 135~GeV \\
    
    \midrule
    
    $m_X$ & 340~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.33 & 0.67
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.10 & 0.21
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.49 & 0.27
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.345 & 0.080
      \end{tabular}
    } \\
    $m_S$ & 145~GeV \\
    
    \midrule
    
    $m_X$ & 340~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.46 & 0.66
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.71 & 0.14
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.59 & 0.27
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.172 & 0.045
      \end{tabular}
    } \\
    $m_S$ & 155~GeV \\
    
    \midrule
    
    $m_X$ & 340~GeV &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        4.49 & 0.66
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.287 & 0.063
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        1.69 & 0.27
      \end{tabular}
    } &
    \multirow{2}{*}{ 
      \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
        0.051 & 0.017
      \end{tabular}
    } \\
    $m_S$ & 165~GeV \\
    
    \midrule
    \midrule
    
    \multicolumn{2}{c}{Background} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      2.31 & 1.39
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      3.00 & 1.78
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      21.12 & 5.18
    \end{tabular} &
    \begin{tabular}{S[table-format=1.4]@{$\pm$}S[table-format=2.4]}
      7.93 & 2.04
    \end{tabular} \\
    
    \midrule
    \midrule
    
    \multicolumn{2}{c}{Observed} & 2 & 3 & 22 & 4 \\
    
    \bottomrule
  \end{tabular}
  \caption{Expected and observed yields after all selection criteria for the $HH$ and $X\rightarrow SS$ searches 
                in the four lepton channel.  The non-resonant $HH$ signal is assumed to have a cross-section of 33.4~fb 
                and the resonant $HH$ and $X\rightarrow SS$ signals are assumed to have a cross-section of 1~pb.  
                The $SS\rightarrow4W\rightarrow4\ell$ branching ratio depends on $m_S$ and ranges from $1.8\times10^{-3}$ 
                to $1.0\times10^{-2}$. Systematic uncertainties in the signal and background yields are shown.}
  \label{tab:yields-4l}
\end{table}



